Nonlinear semigroups for delay equations in Hilbert spaces, inertial manifolds and dimension estimates

We study the well-posedness of nonautonomous nonlinear delay equations in $\mathbb{R}^{n}$ as evolutionary equations in a proper Hilbert space. We present a construction of solving operators (nonautonomous case) or nonlinear semigroups (autonomous case) for a large class of such equations. The main idea can be easily extended for certain PDEs with delay. Our approach has lesser limitations and much more elementary than some previously known constructions of such semigroups and solving operators based on the theory of accretive operators. In the autonomous case we also study differentiability properties of these semigroups in order to apply various dimension estimates using the Hilbert space geometry. However, obtaining effective dimension estimates for delay equations is a nontrivial problem and we explain it by means of a scalar delay equation. We also discuss our adjacent results concerned with inertial manifolds and their construction for delay equations.

==> AuxiliaryLemmas.tex <==
\section{A lemma on the differentiability of Lipschitz mappings}
\label{APP: LipschitzMapsLemmas}
In what follows, $\mathbb{E}$ denotes an arbitrary real Banach space. Since we do not assume that $\mathbb{E}$ satisfies the Radon-Nikodym property (and, in fact, the space $\mathbb{E}$ from Section \ref{SEC: InvariantManifoldsDelay} is the space of continuous functions, for which it is known that this property is not satisfied), it is not a priori known that a Lipschitz function $F \colon \mathbb{R}^{j} \to \mathbb{E}$ is differentiable almost everywhere (see the monograph of J.~Diestel and J.~J.~Uhl \cite{DiestelUhl1977}). For this we will additionally assume that $F$ is Lipschitz as a functions with values in a smaller Hilbert space. Our interest is to apply the lemma below to the function $F:=\Phi$, where $\Phi$ is defined in Section \ref{SEC: InvariantManifoldsDelay}.

\begin{lemma}
	\label{LEM: LipContDiff}
	Let $F \colon \mathbb{R}^{m} \to \mathbb{H}_{aux}$ be a locally Lipschitz function with values in some Hilbert space $\mathbb{H}_{aux}$. Suppose also that $\mathbb{H}_{aux}$ is continuously embedded into $\mathbb{E}$. Let there exist a family of linear maps $D(x) \in \mathcal{L}(\mathbb{R}^{j};\mathbb{E})$, which continuously depend on $x \in \mathbb{R}^{m}$. Let $F'(x)=D(x)$ be satisfied for almost all $x \in \mathbb{R}^{m}$. Then $F \colon \mathbb{R}^{m} \to \mathbb{E}$ is continuously Fr\'{e}chet differentiable and $F'(x)=D(x)$ for all $x \in \mathbb{R}^{m}$.
\end{lemma}
\begin{proof}
	Let us start with the case $j=1$. Since the Hilbert space $\mathbb{H}_{aux}$ satisfies the Radon-Nikodym property, the Lipschitz continuity of $F$ implies its absolute continuity and, consequently (see p. 106 in \cite{DiestelUhl1977}), for all $x \in \mathbb{R}$ we have
	\begin{equation}
	F(x) - F(0) = \int_{0}^{x} F'(y) dy = \int_{0}^{x}D(y)dy.
	\end{equation}
	Since the function on the right-hand side is continuously differentiable with its derivative $D(x)$, the same holds for $F(\cdot)$.
	
	Now let us consider, for simplicity of notation, the case $j=2$ (the case $j>2$ can be treated analogously). Let $\mathcal{D}$ denote the unit disk and $\mathcal{S}^{1}$ denote the unit circle in $\mathbb{R}^{2}$. Our aim is to show that for all $x \in \mathbb{R}^{2}$ there is a dense subset of $\xi \in (\mathcal{S}^{1} + x)$ for which we have $F(x+t \xi) - F(x) = tD(x)\xi + o(t)$ as $t \to 0+$, where $t \in [0,1]$. Without loss of generality, we may assume that $x=0$. Let $\widetilde{D}$ denote the set of all $y \in \mathcal{D}$ for which we have $F'(y)=D(y)$. By assumption, $\lambda_{2}(\widetilde{D}) = \lambda_{2}(\mathcal{D}) = \pi$, where $\lambda_{2}(\cdot)$ denotes the two-dimensional Lebesgue measure. Consider the partition of $\mathcal{D}$ onto closed unit segments $\mathcal{I}_{\alpha}$ by the angle $\alpha \in [0,2\pi]$, i.~e. $\mathcal{I}_{0} := \{ (x_{1},0) \in \mathbb{R}^{2} \ | \ x_{1} \in [0,1] \}$ and $\mathcal{I}_{\alpha}$ is given by the rotation of $\mathcal{I}_{0}$ by $\alpha$. From the Fubini theorem we have
	\begin{equation}
	\label{EQ: LipLemma1Fubini}
	\pi = \lambda_{2}(\widetilde{\mathcal{D}}) = \frac{1}{2} \int_{0}^{2\pi} \lambda_{1}(\mathcal{I}_{\alpha} \cap \widetilde{\mathcal{D}}) d \alpha,
	\end{equation}
	where $\lambda_{1}$ denotes the one-dimensional Lebesgue measure. Consider the set $\mathcal{C}_{k}$ of all $\alpha \in [0,2\pi]$ such that $\lambda_{1}(\mathcal{I}_{\alpha} \cap \widetilde{\mathcal{D}}) \geq 1 - 1/k$. From \eqref{EQ: LipLemma1Fubini} it immediately follows that $\mathcal{C}_{k}$ is a set of full measure in $[0,2\pi]$. Then the set $\bigcap_{k=1}^{\infty}\mathcal{C}_{k}$ is also a set of full measure in $[0,2\pi]$. In particular, there is a dense set of $\alpha \in [0,2\pi]$, for which $F'(y)$ exists and $F'(y)=D(y)$ for almost all $y \in \mathcal{I}_{\alpha}$. Let $\xi_{\alpha} \in \mathcal{I}_{\alpha}$ be the unique unit vector, i.~e. $\mathcal{I}_{\alpha} = \bigcup_{t \in [0,1]} \{ t \xi_{\alpha} \}$. Then for such $\alpha$ the derivative of the Lipschitz function $F_{\alpha}(t) = F(t \xi_{\alpha})$ exists and coincides with $D(t\xi_{\alpha})\xi$ for almost all $t \in [0,1]$. From the previous case ($j=1$) we have that $F_{\alpha}$ is differentiable at $t = 0$ and $F(t \xi_{\alpha}) - F(0) = tD(0)\xi_{\alpha} + o(t)$.
	
	Now we will prove that $F(h)-F(0) = D(0)h + o(h)$ as $h \to 0$. Let $\varepsilon>0$ be fixed. Our aim is to find $\delta>0$ such that for some $C>0$ (independent of $\delta$)
	\begin{equation}
	\|(F(0+h)-F(0) - D(0)h) \|_{\mathbb{E}} \leq C\varepsilon |h|
	\end{equation}
	provided that $|h| < \delta$. Let $\xi_{l}$, where $l=1,2,\ldots,L$ for some $L>0$ be an $\varepsilon$-net on $\mathcal{S}^{1}$ such that $F(t \xi_{l}) - F(0) = tD(0)\xi_{l} + o(t)$ as $t \to 0$ for any $l$. Then we can find $\delta>0$ such that if $|t| < \delta$ then
	\begin{equation}
	\|F(t \xi_{l}) - F(0) - tD(0)\xi_{l}\|_{\mathbb{E}} < \varepsilon |t|.
	\end{equation}
	for all $l$. For any $h \in \mathbb{R}^{2}$ we put $\xi := \frac{h}{|h|}$. Then $h = |h| \xi$, where $\xi \in \mathcal{S}^{1}$. Let $1 \leq l_{0} \leq L$ be such that $|\xi_{l_{0}}-\xi| < \varepsilon$. Since $F$ is Lipschitz and $D(0)$ is bounded, there exists a constant $C>0$ such that
	\begin{equation}
	\begin{split}
	\|(F(h)-F(0) - D(0)h) \|_{\mathbb{E}} \leq \| F(h) - F(|h|\xi_{l_{0}}) \|_{\mathbb{E}} +\\+ \| F(|h|\xi_{l_{0}}) - F(0) - |h|D(0) \xi_{l_{0}} \|_{\mathbb{E}} + \| D(0)(|h|\xi_{l_{0}} - h) \|_{\mathbb{E}} \leq C \varepsilon |h|
	\end{split}
	\end{equation}
	provided that $|h| < \delta$. This gives the desired differentiability at $x=0$. Thus, $F'(x) = D(x)$ for all $x \in \mathbb{R}^{2}$ and the lemma is proved.
\end{proof}

Note that the Lipschitz condition in Lemma \ref{LEM: LipContDiff} is essential. The Cantor staircase function shows that at least the absolute continuity should be required in the case $j=1$. When $j>1$ the proof highly relies on the Lipschitz continuity.

